Dynamics of QCD Matter -- current status

In this article, there are 18 sections discussing various current topics in the field of relativistic heavy-ion collisions and related phenomena, which will serve as a snapshot of the current state of the art. Section 1 reviews experimental results of some recent light-flavored particle production data from ALICE collaboration. Other sections are mostly theoretical in nature. Very strong but transient magnetic field created in relativistic heavy-ion collisions could have important observational consequences. This has generated a lot of theoretical activity in the last decade. Sections 2, 7, 9, 10 and 11 deal with the effects of the magnetic field on the properties of the QCD matter. There are several unanswered questions about the QCD phase diagram. Sections 3, 11 and 18 discuss various aspects of the QCD phase diagram and phase transitions. Recent years have witnessed interesting developments in foundational aspects of hydrodynamics and their application to heavy-ion collisions. Sections 12, 15, 16 and 17 of this article probe some aspects of this exciting field. Transport coefficients together with their temperature- and density-dependence, are essential inputs in hydrodynamical calculations. Sections 5, 8 and 14 deal with calculation/estimation of various transport coefficients (shear and bulk viscosity, thermal conductivity, relaxation times, etc.) of quark matter and hadronic matter. Sections 4, 6 and 13 deals with interesting new developments in the field. Section 4 discusses color dipole gluon distribution function at small transverse momentum in the form of a series of Bells polynomials. Section 6 discusses the properties of Higgs boson in the quark gluon plasma using Higgs-quark interaction. Section 13 discusses modification of coalescence model to incorporate viscous corrections and application of this model.

==> def_file.tex <==
\def\be {\begin{equation}}
\def\ee {\end{equation}}
\def\bea {\begin{eqnarray}}
\def\eea {\end{eqnarray}}
\def\beq{\begin{equation}}   \def\eeq{\end{equation}}
\def\beeq{\begin{eqnarray}} \def\eeeq{\end{eqnarray}}
\def\k {|{\vec k}|}
\def\q {|{\vec q}|}
\def\ks {{|{\vec k}|}^\ast}
\def\qs {|{{\vec q}|}^\ast}
\def\mqs {M_q^\ast}
\def\eqs {E_q^\ast}
\def\eq {E_q}
\def\mks {M_k^\ast}
\def\ek {E_k}
\def\eks {E_k^\ast}
\def\mp {m_\pi}
\newcommand{\bef}{\begin{figure}}
\newcommand{\eef}{\end{figure}}
\newcommand{\ra}{\rightarrow}
\newcommand{\gm}{\gamma^\mu}
\newcommand{\gf}{\gamma^5}
\newcommand{\N}{\bar{N}}
\newcommand{\del}{\partial}
\def\bt{{\bf{\tau}}}
\def\ba{{\bf{a_1}}}
%\def\br{{\bf{\rho}}}
\def\bp{{\bf{\pi}}}
\def\cl{{\cal{L}}}
\def\noi{\noindent}

\def\sq{\hbox {\rlap{$\sqcap$}$\sqcup$}}


\newenvironment{narrow}[2]{%
\begin{list}{}{%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{#1}%
\setlength{\rightmargin}{#2}%
\setlength{\listparindent}{\parindent}%
\setlength{\itemindent}{\parindent}%
\setlength{\parsep}{\parskip}}%
\item[]}{\end{list}}

\newcommand{\pts}{\langle{p_T}^2\rangle}
\newcommand{\kts}{\langle{k_T}^2\rangle}

\newcommand{\non}{\nonumber}
\newcommand{\ave}[1]{\left\langle #1 \right\rangle}
\newcommand{\eqn}[1]{Eq.\,(\ref{#1})}
\newcommand{\MeV}{\hbox{MeV}}
\newcommand{\GeV}{\hbox{GeV}}
\newcommand{\fm}{\hbox{fm}}
\newcommand{\Nch}{N_{\rm ch}}

\def\eq#1{{(\ref{#1})}}
\def\fig#1{{Fig.~\ref{#1}}}
\def\re#1{{Ref.~\cite{#1}}}
\def\order#1{\mathcal{O}{(#1)}}
\def\b#1{\mathbf{#1}}
%


\newcommand{\myack}{\paragraph{Acknowledgements}}

